InstructABSA: Instruction Learning for Aspect Based Sentiment Analysis

We introduce InstructABSA, an instruction learning paradigm for Aspect-Based Sentiment Analysis (ABSA) subtasks. Our method introduces positive, negative, and neutral examples to each training sample, and instruction tune the model (Tk-Instruct) for ABSA subtasks, yielding significant performance improvements. Experimental results on the Sem Eval 2014, 15, and 16 datasets demonstrate that InstructABSA outperforms the previous state-of-the-art (SOTA) approaches on Term Extraction (ATE), Sentiment Classification(ATSC) and Sentiment Pair Extraction (ASPE) subtasks. In particular, InstructABSA outperforms the previous state-of-the-art (SOTA) on the Rest14 ATE subtask by 5.69% points, the Rest15 ATSC subtask by 9.59% points, and the Lapt14 AOPE subtask by 3.37% points, surpassing 7x larger models. We also get competitive results on AOOE, AOPE, and AOSTE subtasks indicating strong generalization ability to all subtasks. Exploring sample efficiency reveals that just 50% train data is required to get competitive results with other instruction tuning approaches. Lastly, we assess the quality of instructions and observe that InstructABSA's performance experiences a decline of ~10% when adding misleading examples.

==> tables/absa1_ate_example.tex <==
\begin{table*}[]
\begin{tabular}{ll}
\hline
\textbf{Task}             & Aspect Term Extraction (ATE)                                                       \\ \hline
\textbf{Model}            & InstructABSA-1                                                                    \\ \hline
\textbf{Definition}       & Definition: The output will be the aspects (both implicit and explicit)           \\
\textbf{}                 & which have an associated opinion that are extracted from the input text.          \\
\textbf{}                 & In cases where there are no aspects the output should be noaspectterm.            \\ \hline
\textbf{Positive Example} & Positive example 1-                                                               \\
\textbf{}                 & input: With the great variety on the menu , I eat here often and never get bored. \\
\textbf{}                 & output: menu                                                                      \\
\textbf{}                 & Positive example 2-                                                               \\
\textbf{}                 & input: Great food, good size menu, great service and an unpretensious setting.    \\
\textbf{}                 & output: food, menu, service, setting                                              \\ \hline
\textbf{}                 & input: My son and his girlfriend both wanted cheeseburgers and they were huge!    \\
                          & output:                                                                           \\ \hline
\textbf{Output}           & cheeseburgers                                                                     \\ \hline
\end{tabular}
\caption{
     Illustrating \name{}-1 instruction prompting for the ATE sub task.}
\end{table*}

==> tables/absa1_atsc_example.tex <==
\begin{table*}[]
\begin{tabular}{ll}
\hline
\textbf{Task}             & Aspect Term Sentiment Classification (ATSC)                                                  \\ \hline
\textbf{Model}            & InstructABSA-1                                                          \\ \hline
\textbf{Definition} & The output will be 'positive' if the aspect identified in the sentence contains a     \\
                    & positive sentiment. If the sentiment of the identified aspect in the input is   \\
\textbf{}           & negative the answer will be 'negative'. Otherwise, the output should be 'neutral'.          \\
\textbf{}           & For the aspects which are classified as noaspectterm, the sentiment is none.                  \\ \hline
\textbf{Positive Example} & Positive example 1-                                                     \\
\textbf{}           & input: With the great variety on the menu , I eat here often and never get bored.\\
\textbf{}           & Aspect: menu\\
\textbf{}                 & output: positive                                                        \\
\textbf{}                 & Positive example 2-                                                     \\
\textbf{}           & input: Great food, good size menu, great service and an unpretensious setting.\\
\textbf{}           & Aspect: food.\\
\textbf{}                 & output: positive                                                        \\ \hline
\textbf{Input}            & Now complete the following example-                                     \\
\textbf{}           & input: My son and his girlfriend both wanted cheeseburgers and they were huge!                 \\
                          & Aspect: cheeseburgers.                                                  \\
                          & output:                                                                 \\ \hline
\textbf{Output}           & positive                                                           \\ \hline
\end{tabular}
\caption{
     Illustrating \name{}-1 instruction prompting for the ATSC sub task.}
\end{table*}

==> tables/absa1_joint_example.tex <==
\begin{table*}[]
\begin{tabular}{ll}
\hline
\textbf{Task}             & Aspect Sentiment Pair Extraction                                                         \\ \hline
\textbf{Model}            & InstructABSA-1                                                     \\ \hline
\textbf{Definition} & Definition: The output will be the aspects (both implicit and explicit) and the aspects \\
                          & sentiment polarity. In cases where there are no aspects the output \\
\textbf{}                 & should be noaspectterm:none.                                       \\ \hline
\textbf{Positive Example} & Positive example 1-                                                \\
\textbf{}           & input: With the great variety on the menu , I eat here often and never get bored.       \\
\textbf{}                 & output: menu:positive                                              \\
\textbf{}                 & Positive example 2-                                                \\
\textbf{}           & input: Great food, good size menu, great service and an unpretensious setting.          \\
\textbf{}                 & output: food:positive                                              \\ \hline
\textbf{Input}            & Now complete the following example-                                \\
\textbf{}                 & input: My son and his girlfriend both wanted cheeseburgers and     \\
                          & they were huge!                                                    \\
                          & output:                                                            \\ \hline
\textbf{Output}           & cheeseburgers:positive                                             \\ \hline
\end{tabular}
\caption{
     Illustrating \name{}-1 instruction prompting for the AOPE subtask.}
\end{table*}

==> tables/ate_all_results.tex <==
\begin{table}[H]
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{l|ccc|ccc}
\hline
\multicolumn{1}{c|}{\textbf{ATE}} & \multicolumn{3}{c|}{\textbf{Lapt14}} & \multicolumn{3}{c}{\textbf{Rest14}} \\ \hline
\textbf{Model}                    & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P}  & \textbf{R}  & \textbf{F1}  \\ \hline
\textbf{Vanilla T5}        & 93.17 & 88.56 & 90.80 & 95.39 & 90.30 & 92.78 \\
\textbf{Model-1} & 93.92 & 89.01 & 91.40 & 94.60 & 90.98 & 92.76 \\
\textbf{Model-2} & 92.84 & 91.76 & 92.30 & 93.49 & 90.75 & 92.10 \\ \hline
\end{tabular}
}
\caption{The overall results that report the precision (P), recall (R), and F1 scores of \name{}-1 and 2 for the ATE subtask. The table also includes the results of a vanilla T5 fine-tuned using instruction-equipped data similar to \name{}-2. } 
\label{tab:app_ate_all}
\end{table}

==> tables/atsc_all_results.tex <==
\begin{table}[H]
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{l|cc|cc}
\hline
\multicolumn{1}{c|}{\textbf{ATSC}} & \multicolumn{2}{c|}{\textbf{Lapt14}} & \multicolumn{2}{c}{\textbf{Rest14}} \\ \hline
\textbf{Model}                     & \textbf{Accuracy}    & \textbf{F1}    & \textbf{Accuracy}      & \textbf{F1}     \\ \hline
\textbf{Vanilla T5}        & 80.04 & 79.98 & 81.38 & 80.39 \\
\textbf{Model-1} & 80.62 & 79.37 & 86.25 & 85.15 \\
\textbf{Model-2} & 81.56 & 80.84 & 85.17 & 84.47 \\ \hline
\end{tabular}
}
\caption{The overall results that report the Accuracy and F1 scores of \name{}-1 and 2 for the ATSC subtask. The table also includes the results of a vanilla T5 fine-tuned using instruction-equipped data similar to \name{}-2. }
\label{tab:app_atsc_all}
\end{table}

==> tables/combined_table.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}
{
\begin{tabular}{lccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{} & \multicolumn{3}{l|}{Lapt14} & \multicolumn{3}{l|}{Rest14} & \multicolumn{3}{l|}{Rest15} & \multicolumn{3}{l}{Rest16} \\ \cline{2-13} 
 & \multicolumn{1}{l}{ATE} & \multicolumn{1}{l}{ATSC} & \multicolumn{1}{l|}{Joint} & \multicolumn{1}{l}{ATE} & \multicolumn{1}{l}{ATSC} & \multicolumn{1}{l|}{Joint} & \multicolumn{1}{l}{ATE} & \multicolumn{1}{l}{ATSC} & \multicolumn{1}{l|}{Joint} & \multicolumn{1}{l}{ATE} & \multicolumn{1}{l}{ATSC} & \multicolumn{1}{l}{Joint} \\ \hline
GPT2${med}$ &82.04 &- &53.55 &75.94 &-  &60.07  &-  &-  &-  &- &- &- \\
GRACE   &87.93  &-  &75.97  &85.45  &-  &78.07  &-  &-  &-  &-  &- &- \\
BARTABSA  &83.52  &-  &67.37  &87.07  &-  &73.56  &75.48  &-  &66.61  &-  &- &-\\
IT-MTL  &76.93  &-  &66.07  &-  &-  &-  &74.03  &-  &67.06  &79.41  &- &74.07 \\
ABSA-DeBERTa &-  &82.76  &- &-  &89.46  &-  &-  &-  &-  &-  &-  &- \\
LSAT-XdeBERTa &-  &86.31  &-  &-  &90.86  &-  &-  &-  &-  &-  &-  &- \\
RACL-BERT &-  &73.91  &-  &-  &81.61  &-  &-  &74.91  &-  &-  &-  &- \\
Dual-MRC  &-  &75.97  &-  &-  &82.04  &-  &-  &73.59  &-  &-  &-  &- \\
SPAN &-  &-  &68.06  &-  &-  &74.92  &-  &-  &-  &-  &-  &- \\ 
GAS &-  &-  &68.64  &-  &-  &77.13  &-  &-  &66.78  &-  &-  &73.64 \\ 
\hline
InstructABSA-1 &$91.40_{\uparrow3.47}$  &$\textbf{88.37}_{\uparrow2.06}$  &- &$\textbf{92.76}_{\uparrow7.31}$  &$87.42_{\downarrow3.44}$  &  &$75.23_{\downarrow0.25}$  &  &  &$\textbf{81.48}_{\uparrow2.07}$  &  & \\
InstructABSA-2 &$92.30_{\uparrow4.37}$  &$85.85_{\downarrow0.46}$  &- &$92.10_{\uparrow6.65}$  &$89.76_{\downarrow1.10}$  &  &$\textbf{76.64}_{\uparrow1.16}$  &  &  &$80.32_{\uparrow0.91}$  &  & \\
\hline
\end{tabular}
}
\caption{ATE subtask results denoting F1 scores. GPT2$_{med}$ (SB1&2 and SB1&4) and GRACE results are from \citet{hosseini-asl-etal-2022-generative} and \citet{luo-etal-2020-grace}.
}
\label{tab:combined_table}
\end{table*}

==> tables/joint_task_all_results.tex <==
\begin{table}[H]
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{l|ccc|ccc}
\hline
\multicolumn{1}{c|}{\textbf{Joint Task}} & \multicolumn{3}{c|}{\textbf{Lapt14}} & \multicolumn{3}{c}{\textbf{Rest14}} \\ \hline
\textbf{Model}                           & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P}  & \textbf{R}  & \textbf{F1}  \\ \hline
\textbf{Vanialla T5}        & 79.73 & 75.09 & 77.34 & 79.71 & 74.98 & 77.27 \\
\textbf{Model-1} & 80.11 & 77.71 & 78.89 & 77.86 & 74.53 & 76.16 \\
\textbf{Model-2} & 80.42 & 78.29 & 79.34 & 82.45 & 76.7  & 79.47 \\ \hline
\end{tabular}
}
\caption{The overall results that report the precision (P), recall (R), and F1 scores of \name{}-1 and 2 for the Joint task. The table also includes the results of a vanilla T5 fine-tuned using instruction-equipped data similar to \name{}-2. }
\label{tab:app_joint_all}
\end{table}
